New perspectives for heavy flavour physics from the lattice

In this talk I want to convey an idea about the perspectives for precise lattice QCD computations. Some emphasis is put on the field of flavour physics, where lattice QCD seems to be needed the most in the quantitative interpretation of present and future experiments (in particular this is the reason for section 4.3). I do not want to discuss the latest numbers but will focus on the principle, the challenges and the perspectives. I mainly address those in the audience who know little about the field and therefore take a bit of a bird's-eye view of the field. So I do not hesitate to also list trivial facts (e.g. section 4.2) and my personal opinion on what is relevant for the future.

==> plots/hqetstrat1.tex <==
\newcommand{\bla}{}
\newcommand{\cbla}{}
\newcommand{\blu}{}
\newcommand{\red}{}
\newcommand{\cred}{}
\newcommand{\cmag}{}
\newcommand{\slat}[1] 
{
\unitlength #1
\linethickness{0.2mm}
\bla\multiput(0,0)(0,2.0){6}{\line( 1, 0){12}}
\bla\multiput(0,0)(2.0,0){6}{\line( 0, 1){12}}
\linethickness{0.4mm}
\multiput(0,2)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){7}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){7}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){12}}
\put(12,0){\blu\line(0,1){12}}
}
\newcommand{\blat}[1] 
{
\unitlength #1
\linethickness{0.2mm}
\bla\multiput(0,0)(0,2.0){12}{\line( 1, 0){24}}
\bla\multiput(0,0)(2.0,0){12}{\line( 0, 1){24}}
\linethickness{0.4mm}
\multiput(0,2)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,14)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,16)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,18)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,20)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,22)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,24)(2.0,0){13}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){13}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){24}}
\put(24,0){\blu\line(0,1){24}}
}

\unitlength 0.2cm
\begin{picture}(35,30)(-5,-3.5)

\scriptsize 
\put(28,11){\blat{0.035cm}}
\put(28,1){\slat{0.07cm}}
\put(12,1){\blat{0.07cm}}
\put(0,1){\slat{0.14cm}}
\put(0,11){\blat{0.14cm}}
\red\put(-4.5,25.0){HQET}
\red\put(-4.0,19.0){$\mb$}
\red\put(-4.0,21.0){$\fb$}
\red\put(-6.0,16.0){(large}
\red\put(-6.0,14.5){ volume)}
\red\put(15.0,-4.0){$a_1=0.025\ldots0.05\,\fm$}
\red\put(-4.0,-4.0){$a_2=0.05\ldots0.1\,\fm$}
\red\put(4.0,-2.0){$\omega_k(a_2)$}
\red\put(14.0,-2.0){$\omega_k(a_1)$}
\red\put(28.0,-2.0){$\omega_k(a_1)$}
\cbla\put(29,10.5){\vector(0,-1){4.0}}
\cbla\put(30.0,7.0){matching}
\cmag\put(28.0,16.0){$\Phiqcd(L_1)$}
\cred\put(28,2){\vector(-1,0){4.5}}
\put(25,3){$\sigma$}
\normalsize
\end{picture}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nic"
%%% TeX-master: "nic"
%%% End: 


==> plots/hqetstrat2.tex <==

\newcommand{\slat}[1] 
{
\unitlength #1
\linethickness{0.2mm}
\bla\multiput(0,0)(0,2.0){6}{\line( 1, 0){12}}
\bla\multiput(0,0)(2.0,0){6}{\line( 0, 1){12}}
\linethickness{0.4mm}
\multiput(0,2)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){7}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){7}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){12}}
\put(12,0){\blu\line(0,1){12}}
}
\newcommand{\blat}[1] 
{
\unitlength #1
\linethickness{0.2mm}
\bla\multiput(0,0)(0,2.0){12}{\line( 1, 0){24}}
\bla\multiput(0,0)(2.0,0){12}{\line( 0, 1){24}}
\linethickness{0.4mm}
\multiput(0,2)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,14)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,16)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,18)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,20)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,22)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,24)(2.0,0){13}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){13}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){24}}
\put(24,0){\blu\line(0,1){24}}
}

\unitlength 0.2cm
\begin{picture}(35,30)(-5,-1.5)


\put(28,11){\blat{0.035cm}}
\put(28,1){\slat{0.07cm}}
\put(12,1){\blat{0.07cm}}
\put(0,1){\slat{0.14cm}}
\put(0,11){\blat{0.14cm}}
\red\put(-4.5,25.0){HQET}
\red\put(-4.0,19.0){$\mb$}
\red\put(-4.0,21.0){$\fb$}
\red\put(-6.0,16.0){(large}
\red\put(-6.0,14.5){ volume)}
\red\put(9.0,-2.0){$\Phihqet(L_2)$}
\red\put(28.0,-2.0){$\Phihqet(L_1)$}
\cbla\put(29,10.5){\vector(0,-1){4.0}}
\cbla\put(30.0,7.0){matching}
\cmag\put(28.0,16.0){$\Phiqcd(L_1)$}
\cred\put(28,2){\vector(-1,0){4.5}}
\put(25,3){$\sigma$}
\end{picture}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nic"
%%% TeX-master: "nic"
%%% End: 


==> plots/hqetstrat2s.tex <==

\newcommand{\slat}[1] 
{
\unitlength #1
\linethickness{0.1mm}
\bla\multiput(0,0)(0,2.0){6}{\line( 1, 0){12}}
\bla\multiput(0,0)(2.0,0){6}{\line( 0, 1){12}}
\linethickness{0.1mm}
\multiput(0,2)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){7}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){7}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){7}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){12}}
\put(12,0){\blu\line(0,1){12}}
}
\newcommand{\blat}[1] 
{
\unitlength #1
\linethickness{0.1mm}
\bla\multiput(0,0)(0,2.0){12}{\line( 1, 0){24}}
\bla\multiput(0,0)(2.0,0){12}{\line( 0, 1){24}}
\linethickness{0.1mm}
\multiput(0,2)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,14)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,16)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,18)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,20)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,22)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,24)(2.0,0){13}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){13}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){24}}
\put(24,0){\blu\line(0,1){24}}
}

\newcommand{\bblat}[1] 
{
\unitlength #1
\linethickness{0.1mm}
\bla\multiput(0,0)(0,1.0){24}{\line( 1, 0){24}}
\bla\multiput(0,0)(1.0,0){24}{\line( 0, 1){24}}
\linethickness{0.1mm}
\multiput(0,2)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,4)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,6)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,8)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,10)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,12)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,14)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,16)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,18)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,20)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,22)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,24)(2.0,0){13}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){13}{\red\circle*{0.2}}
\multiput(0,1)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,3)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,5)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,7)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,9)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,11)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,13)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,15)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,17)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,19)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,21)(2.0,0){13}{\bla\circle*{0.2}}
\multiput(0,23)(2.0,0){13}{\red\circle*{0.2}}
\multiput(0,0)(2.0,0){13}{\red\circle*{0.2}}
\put(0,0){\blu\line(0,1){24}}
\put(24,0){\blu\line(0,1){24}}
}

\unitlength 0.2cm
\begin{picture}(30,12.0)(0,2.5)

\put(0,4){\bblat{0.0175cm}}
\put(0,7){\slat{0.035cm}}
\put(7,4){\blat{0.035cm}}
\put(7,9){\slat{0.070cm}}
\put(17,4){\blat{0.07cm}}
\cmag\put(4,8){\vector(1,-1){3}}
% \put(8.5,10){$\mathbf\sigma$}
\cmag\put(13.5,11){\vector(1,-1){4}}
%\put(28.5,12){$\mathbf\sigma$}
%\cblu
%\put(1, 1.2){$L=L_1$}
%\put(13,1.2){$L=L_2=2\,L_1$}
%\put(34,1.2){$L=L_3=4\,L_1$}
\end{picture}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nic"
%%% End: 

